The SNPR neighbourhood of tree-child networks

Network rearrangement operations like SNPR (SubNet Prune and Regraft), a recent generalisation of rSPR (rooted Subtree Prune and Regraft), induce a metric on phylogenetic networks. To search the space of these networks one important property of these metrics is the sizes of the neighbourhoods, that is, the number of networks reachable by exactly one operation from a given network. In this paper, we present exact expressions for the SNPR neighbourhood of tree-child networks, which depend on both the size and the topology of a network. We furthermore give upper and lower bounds for the minimum and maximum size of such a neighbourhood.

==> config/titleAndAuthor.tex <==
% # specify title authors, affiliations and mails

% ### TITLE ###
\title{The SNPR neighbourhood of \tchi networks}
\date{}

\usepackage{url}
\urldef{\mailsJK}\path|jo.klawitter@gmail.com|


% % # USED FOR PREPRINT
\usepackage{authblk}
% ### AUTHORS ###
\author[ ]{Jonathan Klawitter}
% ### AFFILIATIONS ###
\affil[ ]{Department of Computer Science, University of Auckland, New Zealand}
\renewcommand\Affilfont{\itshape\small}
\affil[ ]{\textit {\mailsJK}}
% /#
